Behavioral Learning of Dish Rinsing and Scrubbing based on Interruptive Direct Teaching Considering Assistance Rate

Robots are expected to manipulate objects in a safe and dexterous way. For example, washing dishes is a dexterous operation that involves scrubbing the dishes with a sponge and rinsing them with water. It is necessary to learn it safely without splashing water and without dropping the dishes. In this study, we propose a safe and dexterous manipulation system. The robot learns a dynamics model of the object by estimating the state of the object and the robot itself, the control input, and the amount of human assistance required (assistance rate) after the human corrects the initial trajectory of the robot's hands by interruptive direct teaching. By backpropagating the error between the estimated and the reference value using the acquired dynamics model, the robot can generate a control input that approaches the reference value, for example, so that human assistance is not required and the dish does not move excessively. This allows for adaptive rinsing and scrubbing of dishes with unknown shapes and properties. As a result, it is possible to generate safe actions that require less human assistance.

==> Makefile <==
##################################################################
#
# LaTeX / PDFLaTeX Makefile
# (c) Tom Bobach
#  modified by T.Nakaoka
#
# Last Modified: 17. Jul 2007
#   Added 2-levels of recursion for include checks
#
# History:
#   9. May 2007     Initial Version
#   29.Nov 2011     modified by T.Nakaoka: add replacing. Ex: maru to comma
#                                          compilation files are now stored in tmp.
#
# Disclaimer:
#   Use at your own risk.
#   I take no responsibility for this Makefile eating up your most
#   precious work, teaching your baby bad language or evoking evil
#   ghosts.
#
# What happens:
#   The current directory is searched for a *.tex file containing
#   the string "\documentclass"; this will be the main file.
#   All files included in the main file via "\include" will be
#   added to the source files.
#   The source files are searched for occurences of strings of the
#   form "{figs/<name>}". For each <name> the first of the
#   following conversion rules that matches is applied
#
#   if the target is a pdf:
#     figs_orig/<name>.png    ->    figs/<name>.png
#     figs_orig/<name>.jpg    ->    figs/<name>.png
#     figs_orig/<name>.eps    ->    figs/<name>.pdf
#     figs_orig/<name>.pdf    ->    figs/<name>.pdf
#     figs_orig/<name>.dia    ->    figs/<name>.pdf
#     figs_orig/<name>.dot    ->    figs/<name>.pdf
#     figs_orig/<name>.svg    ->    figs/<name>.pdf
#     figs_orig/<name>.xcf    ->    figs/<name>.png
#
#   if the target is a dvi / ps:
#     figs_orig/<name>.png    ->    figs/<name>.eps
#     figs_orig/<name>.jpg    ->    figs/<name>.eps
#     figs_orig/<name>.pdf    ->    figs/<name>.eps
#     figs_orig/<name>.eps    ->    figs/<name>.eps
#
#   If any of the input files contains the string "\bibliographystyle",
#   bibtex is invoked, the make dependency linked to the bib file found
#   in the "\bibliography{<file>}" entry.
#
#
# Note on xfig / ps+tex:
#   As some kind of support for xfig / ps+tex, the following conversion
#   takes place:
#     figs_orig/<name>.fig    ->    figs/<name>.eps_t + figs/<name>.{eps|pdf}
#
# Usage:
#   make info        prints some info about the setup, what is considered
#                    the main file, what is the bibliography, what are
#                    the relevant images etc.
#   make clean       removes typical intermediate files.
#   make (pdf)       runs as stated in the beginning, assuming as target
#                    a pdf named after the main file.
#   make open        opens the pdf by gnome-open
#   make watch       checks every second for changes in *.tex, *.bib,
#                    and figs_orig/*
#   make count       counts every character in the generated pdf.
#                    prints TODOs.
#
#
# TODO:
#   - support an arbitrary number of levels of recursion (currently 2)
#   - strip the comments from the texfile for every analysis of the text
#     (currently only done for bib file inclusion)
##################################################################

##################################################################
#   Main definitions - place your customizations here
##################################################################

# latexdiff-git -r b2b786f -t CFONT -e utf8 main.tex
# MAINFILE=main-diffb2b786f.tex
MAINFILE=main.tex
FIGRAW=figs_orig
FIGDIR=figs

TMPDIR=tmp
SUBDIR=chapter

# uncomment the following to have the images rescaled
#CONVERT=convert -geometry 200
CONVERT=convert

ifeq ($(shell uname),Darwin)
	OPEN=open
else
	OPEN=gnome-open
endif

# upload settings
UPLOAD_USER=$(SSH_USER)
UPLOAD_DIR=/home/jsk/$(UPLOAD_USER)/public_html/pdf
UPLOAD_LATEST_DIR=/home/jsk/$(UPLOAD_USER)/public_html/pdf
UPLOAD_PREFIX=$(UPLOAD_USER)-mthesis-
UPLOAD_TIME=$(shell date +%s)
UPLOAD_SERVER=www

UPLOAD_PATH=$(UPLOAD_DIR)/$(UPLOAD_PREFIX)$(UPLOAD_TIME).pdf
UPLOAD_LATEST_PATH=$(UPLOAD_LATEST_DIR)/$(UPLOAD_PREFIX)latest.pdf


##################################################################
#   Some Definitions that should not need change
##################################################################

ifneq ($(words $(MAINFILE)),1)
$(error For automatic main file detection, only one .tex file can contain the "\documentclass" string. run make MAINFILE=<your mainfile>)
endif
# Currently, only two levels of recursion for included input is supported.
# If you need more, extend as you like after the scheme below.
TEXFILESPRE:=\
  $(shell grep "\\\\include{" $(MAINFILE) | sed 's/.*{\([^}]*\)}.*/\1/g') \
  $(shell egrep "\\\\input{.*\.tex}" $(MAINFILE) | sed 's/.*{\([^}]*\).tex}.*/\1/g')

ifneq ($(words $(TEXFILESPRE)),0)
  TEXFILES:=\
    $(MAINFILE:.tex=)\
    $(TEXFILESPRE)\
    $(shell grep "\\\\include{" $(TEXFILESPRE:=.tex) | sed 's/.*{\([^}]*\)}.*/\1/g') \
    $(shell egrep "\\\\input{.*\.tex}" $(TEXFILESPRE:=.tex) | sed 's/.*{\([^}]*\).tex}.*/\1/g')
else
  TEXFILES:=$(MAINFILE:.tex=) $(TEXFILESPRE)
endif


MUTE=@
#MUTE=
SILENT=> /dev/null
#SILENT=
VERYSILENT=1> /dev/null 2>/dev/null

MAKE=make --no-print-directory
LS=ls -1 --color=none
CP=cp

LATEX=./scripts/platex.sh
BIBTEX=./scripts/bibtex.sh
EXTRACT_BOUNDINGBOX=extractbb

MSG_LAB_CHANGED="LaTeX Warning: Label(s) may have changed"
MSG_REF_UNDEFINED="LaTeX Warning: Reference.*undefined on input line.*"
MSG_CIT_UNDEFINED="LaTeX Warning: Citation.*undefined on input"

# strip all comments and extract the bibliography
FIND_BIB_FILE=$(shell \
	sed -e "s/\\\\%//g" $(1) | \
	sed -e "s/\([^%]*\).*/\1/g" | \
	grep "\\\\bibliography{"  | \
        sed 's/.*{\([^}^ ]*\)}.*/\1/g').bib

BIBFILE:=$(call FIND_BIB_FILE, $(TEXFILES:=.tex))
ifneq ($(BIBFILE),.bib)
  ifneq ($(wildcard *.bib),)
    BBL:=$(MAINFILE:.tex=.bbl)
  else
    BBL:=$(BIBFILE)
  endif
else
  BBL:=$(BIBFILE)
endif

##################################################################
#   The figures used in the tex file
##################################################################

# Extract all lines that address the figures directory somehow
FIGS=$(sort $(shell grep -e $(FIGDIR)/ $(TEXFILES:=.tex) \
		    | sed "s/.*{$(FIGDIR)\/\([^}]*\).*/\1/g" ))

# the standard conversion rules are those, for postscript
# that changes into all->eps
EPS_TO=.pdf
PDF_TO=.pdf
PNG_TO=.png
JPG_TO=.jpg
DIA_TO=.pdf
SVG_TO=.pdf
DOT_TO=.pdf
XCF_TO=.png

# Find all existing files of a certain type in FIGRAW that would
# -after conversion- be included from FIGDIR
FIGSRCEPS=$(wildcard $(addprefix $(FIGRAW)/, $(addsuffix .eps, $(FIGS))))
FIGSRCJPG=$(wildcard $(addprefix $(FIGRAW)/, $(addsuffix .jpg, $(FIGS))))
FIGSRCPNG=$(wildcard $(addprefix $(FIGRAW)/, $(addsuffix .png, $(FIGS))))
FIGSRCPDF=$(wildcard $(addprefix $(FIGRAW)/, $(addsuffix .pdf, $(FIGS))))
FIGSRCDIA=$(wildcard $(addprefix $(FIGRAW)/, $(addsuffix .dia, $(FIGS))))
FIGSRCSVG=$(wildcard $(addprefix $(FIGRAW)/, $(addsuffix .svg, $(FIGS))))
FIGSRCDOT=$(wildcard $(addprefix $(FIGRAW)/, $(addsuffix .dot, $(FIGS))))
FIGSRCXCF=$(wildcard $(addprefix $(FIGRAW)/, $(addsuffix .xcf, $(FIGS))))
FIGSRCEPST=$(wildcard $(addprefix $(FIGRAW)/, $(FIGS:.eps_t=.fig)))

# Set up all the targets that should be created in the FIGDIR
FIGDEPEPS=$(subst $(FIGRAW)/, $(FIGDIR)/, $(FIGSRCEPS:.eps=$(EPS_TO)))
FIGDEPJPG=$(subst $(FIGRAW)/, $(FIGDIR)/, $(FIGSRCJPG:.jpg=$(JPG_TO)))
FIGDEPPNG=$(subst $(FIGRAW)/, $(FIGDIR)/, $(FIGSRCPNG:.png=$(PNG_TO)))
FIGDEPPDF=$(subst $(FIGRAW)/, $(FIGDIR)/, $(FIGSRCPDF:.	pdf=$(PDF_TO)))
FIGDEPDIA=$(subst $(FIGRAW)/, $(FIGDIR)/, $(FIGSRCDIA:.dia=$(DIA_TO)))
FIGDEPSVG=$(subst $(FIGRAW)/, $(FIGDIR)/, $(FIGSRCSVG:.svg=$(SVG_TO)))
FIGDEPDOT=$(subst $(FIGRAW)/, $(FIGDIR)/, $(FIGSRCDOT:.dot=$(DOT_TO)))
FIGDEPXCF=$(subst $(FIGRAW)/, $(FIGDIR)/, $(FIGSRCXCF:.xcf=$(XCF_TO)))
FIGDEPEPST=$(subst $(FIGRAW)/, $(FIGDIR)/, $(FIGSRCEPST:.fig=.eps_t))

ALLFIGSRC=$(FIGSRCJPG) $(FIGSRCPNG) $(FIGSRCPDF) $(FIGSRCEPST) $(FIGSRCEPS) $(FIGSRCDIA) $(FIGSRCSVG) $(FIGSRCDOT) $(FIGSRCXCF)
ALLFIGS=$(FIGDEPJPG) $(FIGDEPPNG) $(FIGDEPPDF) $(FIGDEPEPST) $(FIGDEPEPS) $(FIGDEPDIA) $(FIGDEPSVG) $(FIGDEPDOT) $(FIGDEPXCF)
FIGSUBDIRS := $(shell find ${FIGRAW} -type d -print | sed "s/$(FIGRAW)/$(FIGDIR)/g")

##################################################################
#   All the shell magic that helps us manage the twisted LaTeX
#   Compilation procedure
##################################################################


clear_valid=( [ ! -e .valid ] || $(RM) .valid )
check_undef_citations=\
  ( egrep $(MSG_CIT_UNDEFINED) $(TMPDIR)/$(MAINFILE:.tex=.log) > /dev/null )

# determine the changeset for citations
define check_citationchange
	(                                                \
	  [ -e .citations ] || touch .citations ;        \
	  ( grep "\\citation" $(TMPDIR)/$(MAINFILE:.tex=.aux)      \
		| sort                                   \
		| uniq                                   \
		| diff .citations -                      \
		> .citediff                              \
	  )                                              \
	)
endef

# exctract the citations from the aux file
define make_citations
	(                                                   \
	  (                                                 \
	    [ -e $(TMPDIR)/$(MAINFILE:.tex=.aux) ] &&                 \
	    ( echo "[info] Extracting citations...";        \
		grep "\\citation" $(TMPDIR)/*.aux     \
		| sort                                      \
		| uniq                                      \
		> .citations                                \
	    )                                               \
	  )                                                 \
	  || touch .citations                               \
	)
endef

# comparing the citations in $(MAINFILE:.tex=.aux)
# against those in .citations.
# if there are differences, .citediff is changed.
define make_citediff
	(                                                     \
	  ( [ -e .citations ] || touch .citations ;           \
	    [ -e .citediff  ] || touch .citediff ;            \
	    echo "[info] Checking for changed Citations..." ; \
	    grep "\\citation" $(TMPDIR)/*.aux           \
		| sort                                        \
		| uniq                                        \
		| diff .citations -                           \
	    > .citediff__                                     \
	  )                                                   \
	  || mv .citediff__ .citediff                         \
	)
endef

# compiles the document
# the file .valid is created if the compilation went without
# errors
define runtexonce
  ( 	                                                    \
    $(clear_valid);                                         \
    ( $(LATEX) $(MAINFILE) $(SILENT) &&                     \
      touch .valid );                                       \
    (                                                       \
      ( egrep $(MSG_REF_UNDEFINED) $(TMPDIR)/$(MAINFILE:.tex=.log)    \
        > .undefref ) ;                                     \
      ( egrep $(MSG_CIT_UNDEFINED) $(TMPDIR)/$(MAINFILE:.tex=.log)    \
        > .undefcit ) ;                                     \
      true                                                  \
    )                                                       \
  )
endef

# compile the document as many times as necessary to
# have cross-references right
define runtex
(                                                                      \
  echo "[info] Running tex...";                                        \
  $(runtexonce);                                                       \
  while( grep $(MSG_LAB_CHANGED) $(TMPDIR)/$(MAINFILE:.tex=.log) > /dev/null ) ; \
  do                                                                   \
      echo "[info] Rerunning tex...";                                  \
      $(runtexonce);                                                   \
  done                                                                 \
)
endef

##################################################################
#   Main compilation rules
##################################################################

pdf: $(MAINFILE:.tex=.pdf)

ps:  $(MAINFILE:.tex=.dvi)

dvi: $(MAINFILE:.tex=.ps)



$(MAINFILE:.tex=.pdf): $(TMPDIR)/$(MAINFILE:.tex=.pdf)
	$(MUTE)cd $(TMPDIR) && cp $(MAINFILE:.tex=.pdf) ../
	$(MUTE)echo "[info] Created PDF."

$(TMPDIR)/$(MAINFILE:.tex=.pdf): $(TMPDIR)/docinfo.out .compilesource
	# $(MUTE)cd $(TMPDIR) && ../scripts/out2uni $(MAINFILE:.tex=)
	$(MUTE)$(runtex)
	$(MUTE)cd $(TMPDIR) && dvipdfmx -V 5 $(MAINFILE:.tex=.dvi)

$(TMPDIR)/docinfo.out: scripts/out2uni docinfo.txt
	$(MUTE)[ -d $(TMPDIR) ] || mkdir $(TMPDIR)
	$(MUTE)cp docinfo.txt $(TMPDIR)/docinfo.out
	$(MUTE)nkf -e --overwrite $(TMPDIR)/docinfo.out
	# $(MUTE)scripts/out2uni $(TMPDIR)/docinfo.out

scripts/out2uni: scripts/out2uni.c
	$(MUTE)cd scripts && $(CC) -DEUC -o out2uni out2uni.c

# the dvi creation path invokes standard tex and requires other figures
$(MAINFILE:.tex=.dvi): .force
	$(MUTE)echo "not implemented now."
	#$(MUTE)$(MAKE) .compilesource \
		LATEX="platex -shell-escape -interaction=nonstopmode" \
		EPS_TO=.eps \
		PDF_TO=.eps \
		PNG_TO=.eps \
		JPG_TO=.eps \
		DIA_TO=.eps \
		SVG_TO=.eps \
		DOT_TO=.eps \
		XCF_TO=.eps

%.ps: %.dvi
	$(MUTE)echo "[info] Converting DVI to PS"
	$(MUTE)dvips $< -o $@ $(VERYSILENT)

.compilesource: .force
	$(MUTE)$(MAKE) .valid
	$(MUTE)[ -z "$(BBL)" ] || $(MAKE) .citations
	$(MUTE)[ -e .valid ] || (                                    \
	  ( [ -e .compiled ] || $(MAKE) .compiled ) ;                \
	  ( [ -e .compiled ] || $(MAKE) .compiled ) ;                \
	  ( [ -e .compiled ] || $(MAKE) .compiled ) ;                \
	  ( [ -e .compiled ] || echo "[Error] Could not make it work after 3 runs. Weird." ) \
	)
	$(MUTE) (                                                    \
           echo ; echo "Compilation Warnings:" ;                     \
	   grep "Warning" $(TMPDIR)/$(MAINFILE:.tex=.log) ;                    \
	   grep "Error" $(TMPDIR)/$(MAINFILE:.tex=.log) ;                      \
	   grep -A 1 "Undefined" $(TMPDIR)/$(MAINFILE:.tex=.log) || true       \
	)
	$(MUTE)[ ! -e $(TMPDIR)/$(MAINFILE:.tex=.bbl) ] || (                   \
	  echo ; echo "Bibtex Warnings:" ;                           \
	  grep "Warning" $(TMPDIR)/$(MAINFILE:.tex=.blg) ;                     \
	  grep "Error" $(TMPDIR)/$(MAINFILE:.tex=.blg) || true                 \
	)
	$(MUTE)[ -z "$(TMPDIR)/$(BBL)" -a -e .valid ] || [ -n "$(TMPDIR)/$(BBL)" -a -e .compiled ]

.figs: makefigdir $(ALLFIGS)
	$(MUTE)touch .figs

makefigdir:
	$(MUTE)mkdir -p $(FIGSUBDIRS)

clean:
	$(MUTE)$(RM) *.bbl *.blg *.aux *.log *.pbm *.fls *.toc *.out
	$(MUTE)$(RM) -r $(TMPDIR)/*
	$(MUTE)$(RM) *.*~
	$(MUTE)$(RM) .citations .citediff* .compiled .figs .undefcit .undefref .valid
	$(MUTE)for i in $(TEXFILES:=.tex) $(BIBFILE) ; do \
		$(RM) .$$i; \
	done;
#added
	$(MUTE)$(RM) $(SUBDIR)/*~
	$(MUTE)$(RM) *~
	$(MUTE)$(RM) -r .$(SUBDIR)

figclean:
	$(MUTE)$(RM) -r $(FIGDIR)/*
	$(MUTE)find $(FIGDIR) -type f ! -name .gitkeep | xargs $(RM)

distclean: clean figclean
	$(MUTE)$(RM) $(MAINFILE:.tex=.ps) $(MAINFILE:.tex=.dvi) $(MAINFILE:.tex=.pdf)

open: $(MAINFILE:.tex=.pdf)
	$(OPEN) $<

view: $(MAINFILE:.tex=.pdf)
	kpdf $< > /dev/null 2>&1 &

viewdvi: $(MAINFILE:.tex=.dvi)
	kdvi $(<:.dvi=) > /dev/null 2>&1 &

viewps: $(MAINFILE:.tex=.ps)
	kghostview $< > /dev/null 2>&1 &

info:
	@echo Main file:    $(MAINFILE)
	@echo Input files:  $(TEXFILES:=.tex)
	@echo Bibliography: $(BIBFILE)
	@echo tmp dir:      $(TMPDIR)
	@echo fig subdir:   $(FIGSUBDIRS)
	@echo Images USED
	@echo
	@echo $(ALLFIGSRC)
	@echo
	@echo Images NOT used
	@echo
	@echo $(filter-out $(ALLFIGSRC), $(wildcard $(FIGRAW)/*))

# just do one run...
.valid: .figs $(TEXFILES:=.tex)
	$(MUTE)$(runtex)

# if citations changed since last run of bibtex, run it again.
.citations: .citediff $(BIBFILE)
	$(MUTE)[ ! -e .compiled ] || rm .compiled
	$(MUTE)(                         \
	  echo "[info] Running BibTex" ; \
	  $(BIBTEX) $(MAINFILE:.tex=) $(SILENT)         \
	) && $(make_citations)
	$(MUTE) $(clear_valid)

.citediff: .force
	$(MUTE)$(make_citediff)

# run as long as necessary
.compiled: $(TEXFILES:=.tex) $(TMPDIR)/$(BBL) .figs
	$(MUTE)echo "Found undefined Citations, rerunning..."
	$(MUTE)$(runtex)
	$(MUTE)$(check_undef_citations) || touch .compiled

.force:



##################################################################
#   Rules to convert the figures into the format that (pdf)latex
#   understands
##################################################################

$(FIGDIR)/%.eps : $(FIGRAW)/%.png
	$(CONVERT) $< $@

$(FIGDIR)/%.eps : $(FIGRAW)/%.jpg
	$(CONVERT) $< $@

$(FIGDIR)/%.eps : $(FIGRAW)/%.dia
	dia -e $@ $<

$(FIGDIR)/%.eps : $(FIGRAW)/%.svg
	inkscape -C -z -E $@ $<

$(FIGDIR)/%.eps : $(FIGRAW)/%.dot
	dot -Tps:cairo $< -o $@

$(FIGDIR)/%.png : $(FIGRAW)/%.xcf
	xcf2png $< > $@
	$(EXTRACT_BOUNDINGBOX) $@

$(FIGDIR)/%.eps : $(FIGRAW)/%.pdf
	$(CONVERT) $< $@

$(FIGDIR)/%.eps : $(FIGRAW)/%.eps
	$(CP) $< $@


$(FIGDIR)/%.png : $(FIGRAW)/%.png
	$(CONVERT) $< $@
	$(EXTRACT_BOUNDINGBOX) $@

$(FIGDIR)/%.jpg : $(FIGRAW)/%.jpg
	$(CONVERT) $< $@
	$(EXTRACT_BOUNDINGBOX) $@

$(FIGDIR)/%.pdf : $(FIGRAW)/%.eps
	ps2pdf -dEPSCrop $< $@
	$(EXTRACT_BOUNDINGBOX) $@

$(FIGDIR)/%.pdf : $(FIGRAW)/%.dia
	dia -e $(FIGDIR)/$*.eps $< ; ps2pdf -dEPSCrop $(FIGDIR)/$*.eps $@
	$(EXTRACT_BOUNDINGBOX) $@

$(FIGDIR)/%.pdf : $(FIGRAW)/%.svg
#	inkscape -C -z -E $(FIGDIR)/$*.eps $< ; ps2pdf -dEPSCrop $(FIGDIR)/$*.eps $@
	rsvg-convert -f pdf -o $@ $<
	$(EXTRACT_BOUNDINGBOX) $@

$(FIGDIR)/%.pdf : $(FIGRAW)/%.dot
#	dot -Tps:cairo $< -o $(FIGDIR)/$*.eps ; ps2pdf -dEPSCrop $(FIGDIR)/$*.eps $@
	dot -Tpdf:cairo $< -o $@
	$(EXTRACT_BOUNDINGBOX) $@

$(FIGDIR)/%.pdf : $(FIGRAW)/%.pdf
	$(CP) $< $@
	$(EXTRACT_BOUNDINGBOX) $@

$(FIGDEPEPST): $(FIGDIR)/%.eps_t : $(FIGRAW)/%.fig
	#fig2dev -L pstex_t -p $(@:.eps_t=) $? > $@
	#fig2dev -L pstex $? $(if $(filter .eps,$(EPS_TO)),,| epstopdf -filter) > ${@:.eps_t=$(EPS_TO)}

watch:
	$(MUTE)[ -d .$(SUBDIR) ] || mkdir .$(SUBDIR)
	$(MUTE)CHANGE=true &&                            \
	while true ; do                                  \
          if $$CHANGE ; then                             \
	    for i in $(TEXFILES:=.tex) $(BIBFILE) ; do   \
	      touch .$$i -r $$i;                         \
	    done;                                        \
	    for i in `( cd $(FIGRAW); ls -1 *.* )` ; do  \
	      touch $(FIGRAW)/.$$i -r $(FIGRAW)/$$i;     \
	    done;                                        \
	    CHANGE=false;                                \
	    make;                                        \
          fi;                                            \
          sleep 1;                                       \
          for i in $(TEXFILES:=.tex) $(BIBFILE) ; do     \
	    if [ .$$i -ot $$i ] ; then                   \
	      CHANGE=true;                               \
	    fi                                           \
          done ;                                         \
          for i in `( cd $(FIGRAW); ls -1 *.* )` ; do    \
	    if [ $(FIGRAW)/.$$i -ot $(FIGRAW)/$$i ] ; then \
	      CHANGE=true;                               \
	    fi                                           \
          done                                           \
        done

count: $(MAINFILE:.tex=.pdf)
	$(MUTE)echo '%%%%%%%%%%%%%%%%%%%%%%%%%%%'
	$(MUTE)echo -n 'characters: '
	$(MUTE)pdftotext main.pdf - | sed -e 's/[ ，．]//g' | wc -m
	$(MUTE)grep '\TODO{' *.tex || echo 'There is nothing to do!!'

compress: $(MAINFILE:.tex=)_s.pdf

$(MAINFILE:.tex=)_s.pdf: $(MAINFILE:.tex=.pdf)
	$(MUTE)gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dNOPAUSE -dQUIET -dBATCH -sOutputFile=.$(MAINFILE:.tex=)_gs.pdf $<
	$(MUTE)pdftk .$(MAINFILE:.tex=)_gs.pdf output .$(MAINFILE:.tex=)_pdftk.pdf compress
	$(MUTE)pdfopt .$(MAINFILE:.tex=)_pdftk.pdf $(MAINFILE:.tex=)_s.pdf
	$(MUTE)rm -f .$(MAINFILE:.tex=)_gs.pdf .$(MAINFILE:.tex=)_pdftk.pdf

UPLOAD_TIME=$(shell date +%s)
upload: $(MAINFILE:.tex=)_s.pdf
	scp $< $(UPLOAD_SERVER):$(UPLOAD_PATH)
	ssh $(UPLOAD_SERVER) chmod o+r $(UPLOAD_PATH)
	ssh $(UPLOAD_SERVER) ln -sf $(UPLOAD_PATH) $(UPLOAD_LATEST_PATH)


==> src/acknowledge.tex <==
\section*{Acknowledgement}

Acknowledgement


==> src/overview.tex <==
\section{Overview}

Overview

